Asynchronism in Cellular Automata

This study introduces Skewed Fully Asynchronous Cellular Automata (SACA), a novel update scheme in cellular automata that updates the states of only two consecutive and adjacent cells, such as ci and ci+1, simultaneously at each time step. The behavior and dynamics of elementary cellular automata (ECA) under this scheme are analyzed and compared with those of synchronous and fully asynchronous update methods. The comparative analysis highlights a range of phenomena, including transitions in ECAs from convergent or non-reversible dynamics to reversible, divergent behavior. The divisibility of lattice size by 2 or 4 is shown to have significant effects on the system dynamics, linked to the presence or absence of atomicity. The study also explores the convergence of ECAs to all-zero or all-one point attractors under SACA, providing theoretical insights that align with experimental findings. Additionally, the research investigates the application of fully asynchronous cellular automata in solving clustering problems. Clustering is defined as grouping objects with similar properties. The proposed method employs reversible asynchronous cellular automata to merge clusters iteratively based on their closeness, continuing until the desired number of clusters is achieved. This approach leverages a small set of rules, leading to faster convergence and efficiency in clustering tasks. The findings underscore the potential of asynchronous cellular automata as a versatile and effective framework for studying complex system dynamics and solving practical problems such as clustering.

==> declaration.tex <==
\begin{center}
\vspace{-5.5cm}
 \textbf{\Large DECLARATION}
\end{center}

%\\
%\\
\def \repauthor{Virendra Kumar Gautam}
\def \repregno{Reg No. - 2022ITM008}
\def \repdegree{Master of Technology}
\def \repbranch{Information Technology}
\def \repstream{}
\def \repcollege{Indian Institute of Engineering Science And Technology}
\def \repplace{P.O. - Botanic Garden, Howrah, West Bengal 711103}
\def \repsupervisor{Dr. Sukanta Das} 
\def \repuniversity{IIEST}
\def \repdate{\today} 
%\justify 
%\setstretch{1.5}
I undersigned hereby declare that the report titled \textbf{Asynchronism in Cellular Automata and Computability}, submitted in partial fulfillment of the requirements for the award of degree of \repdegree\, of the \repuniversity, Shibpur is a bonafide work done by me under supervision of \repsupervisor. This submission represents my ideas in my own words and where ideas or words of others have been included, I have adequately and accurately cited and referenced the original sources. I also declare that I have adhered to ethics of academic honesty and integrity and have not misrepresented or fabricated any data or idea or fact or source in my submission. I understand that any violation of the above will be a cause for disciplinary action by the institute and/or the University and can also evoke penal action from the sources which have thus not been properly cited or from whom proper permission has not been obtained. This report has not been previously formed the basis for the award of any degree, diploma or similar title of any other University. 

\vspace{7cm} % Modify this to any value that pleases your eyes
\begin{flushleft}                           
	Place: \repplace \break
	Date: \today 
	\hfill \repauthor % Keep the student name on same line but right-justify
\end{flushleft}
\newpage

